Point-Pattern Matching Technique for Local Structural Analysis in Condensed Matter

The local arrangement of atoms is one of the most important predictors of mechanical and functional properties of materials. However, algorithms for identifying the geometrical arrangements of atoms in complex materials systems are lacking. To address this challenge, we present a point-pattern matching algorithm that can detect instances of a `template' structure in a given set of atom coordinates. To our knowledge this is the first geometrical comparison technique for atomistic configurations with very different number of atoms, and when the optimal rotations and translations required to align the configurations are unknown. The pattern matching algorithm can be combined with an appropriate set of metrics to quantify the similarity or dissimilarity between configurations of atoms. We demonstrate the unique capabilities of the point-pattern matching algorithm using two examples where the automated analysis of local atomistic structure can help advance the understanding of structure-property relationships in material science: (a) identifying local three-dimensional polyhedral units along interfacial defects, and (b) the analysis of quasi-icosahedral topologies in the atomistic structure of metallic glasses. We anticipate that the pattern matching algorithm will be applicable in the analysis of atomistic structures in broad areas of condensed matter systems, including biological molecules, polymers and disordered metallic systems. An online implementation of the algorithm is provided via the open source code hosted on GitHub (https://github.com/spatala/ppm3d).

==> figures.tex <==
\section*{Figure Legends}

\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.55]{s5_0_-2_1_split.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_1.png}
  \caption{An illustration of the VV-clustering algorithm for identifying the polyhedral unit structure of the $\Sigma5 (0\, \overline{2}\, 1)$ GB. \colb{In (a), the minimum energy atomistic structure (at 0K) of the GB, generated using OVITO \cite{stukowski2009visualization}, is shown along the tilt axis $[\overline{1}\, 0 \, 0]$, where the atoms are colored according to their centro-symmetry parameter.  In (b) and (f), atomistic structure of the GB along with the Voronoi vertices and VV-spheres are shown, as viewed along the tilt axis $[\overline{1}\, 0 \, 0]$ and the boundary-plane normal $[0 \, \overline{2} \, 1]$, respectively. All the Voronoi vertices of overlapping VV-spheres are clustered together and, in (e, i), the polyhedral unit obtained by combining the tetrahedra that correspond to the Voronoi vertices in each cluster is shown. The polyhedron contains thirteen atoms.  In (c) and (g), the polyhedral unit model of the $\Sigma5 (0\, \overline{2}\, 1)$ along the tilt axis $[\overline{1}\, 0 \, 0]$ and the boundary-plane normal $[0 \, \overline{2} \, 1]$, respectively, are shown. The overlapping VV-spheres that classify the void structure are also shown. In (e, ii), the polyhedral units obtained after the post-processing steps are shown and in (d) and (h), the structure of the GB, represented using the split units (Octadecahedra and tetrahedra), is illustrated. This structure reveals the similarity between the two $[1\, 0\ 0]$ symmetric tilt GBs - the $\Sigma5 (0\, \overline{2}\, 1)$ and $\Sigma5 (0\, \overline{1}\, 3)$ (which is shown in Figure S23).}}
  \label{fig:s5a}
\end{figure}

% Due to the translational symmetry of the GB, the unit-cell contains only one polyhedral unit, which is highlighted.

\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.65]{s49_1_1_1_twist.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_2.png}
  \caption{\colb{The polyhedral unit model of the $\Sigma 49 (1 \, 1 \, 1)$ GB, as viewed along the twist-axis $[1 \, 1 \, 1]$, is shown. The symmetric twist GB contains a network of screw dislocations. The core-region of the dislocation is described by the snub-disphenoid units and the atoms at the intersection of the screw dislocations are described by the $14$-atom polyhedral unit. The smallest asymmetric unit (GB unit-cell) is shown and the polyhedral units in the unit-cell are highlighted.}}
  \label{fig:s49twist}
\end{figure}


\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.75]{S3_2_-1_-1.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_3.png}
  \caption{The polyhedral unit model of the $\Sigma 3 (2 \, \overline{1} \, \overline{1})$ GB is illustrated. In (a) and (c), the atomistic structure and the polyhedral units (CTPs, dual-tetrahedra and distorted octahedra) of the symmetric-tilt GB, along the tilt axis $[0\, \overline{1}\, 1]$ and the plane normal $[2 \, \overline{1} \, \overline{1}]$, are shown. The polyhedral units corresponding to the smallest asymmetric unit (the unit-cell) are highlighted. In (b), the unit-cell polyhedral units, along with the overlapping VV-spheres (Bernal holes) and the clusters of atoms that correspond to the polyhedral units, are shown.}
  \label{fig:s3a}
\end{figure}


\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.85]{s3_1_0_-1.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_4.png}
  \caption{The polyhedral unit model of the $\Sigma 3 (1\, 0 \, \overline{1})$ asymmetric tilt GB is illustrated. In (a) and (b), the atomistic structure and the polyhedral units, along the tilt axis $[1 \overline{2}\, 1]$ and the plane normal $[1\, 0 \, \overline{1}]$, are shown. The polyhedral units corresponding to the smallest asymmetric unit (the unit-cell) are highlighted. In (c), the unit-cell polyhedral units, along with the overlapping VV-spheres (Bernal holes) and the clusters of atoms that correspond to the polyhedral units, are shown.}
  \label{fig:s3b}
\end{figure}

\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.75]{S3_faceting.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_5.png}
  \caption{The polyhedral unit structures of the $\Sigma 3$ asymmetric tilt GBs, with the $[0\, 1\, \overline{1}]$ tilt axis, are shown.  The order of the GBs are as follows: (a) $\Sigma 3 (1\, 1\, 1)$, (b) $\Sigma3(11\,5\,5)$, (c) $\Sigma3(4\, 1\, 1)$, (d) $\Sigma3(1\, 0 \,0)$, (e) $\Sigma3(7\, \overline{2} \, \overline{2})$, (f) $\Sigma3(13\, \overline{5} \, \overline{5})$, and (g) $\Sigma3(2 \, \overline{1} \, \overline{1})$. The faceting model is apparent in the GBs shown in (b) and (c), which contain polyhedral units of both the $\Sigma 3 (1\, 1\, 1)$ and $\Sigma3(2 \, \overline{1} \, \overline{1})$ GBs. In (d), (e) and (f), while there are no twin facets, deviations in boundary-plane orientations are accommodated through the shuffling of CTP units, as discussed in section \ref{sec:Results}.}
  \label{fig:s3facet}
\end{figure}

\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.85]{s3_9_-4_-5.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_6.png}
  \caption{The polyhedral unit model of the $\Sigma 3 (9\, \overline{4} \, \overline{5})$ asymmetric tilt GB is illustrated. In (a) and (b), the atomistic structure along with the polyhedral units are shown. The vector $\vec{t}_1 = [1\, 1\, 1]$ is the tilt axis, $\hat{n} = [9\, \overline{4} \, \overline{5}]$ is the BPl normal and $\vec{t}_2 = [\overline{1}\, 14 \, \overline{13}]$.  This GB is vicinal to the $\Sigma3 (2 \, \overline{1}\, \overline{1})$ symmetric tilt GB.  Therefore it contains facets of the CTP units and two polyhedral units (colored in blue and orange) that are a part of the ledge in the vicinal GB.  In (c), the same GB is shown along the $[0 \, \overline{1}\, 1]$ axis, without the dual-tetrahedral units, to emphasize the polyhedral units along the ledge.  In (d), the polyhedral units that belong to the ledge and the clusters of atoms that correspond to these units are shown.}
  \label{fig:s3c}
\end{figure}

\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.65]{S3_18_9_8.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_7.png}
  \caption{The polyhedral unit model of the $\Sigma 3 (18\, 9 \, 8)$ general GB is illustrated. In (a) and (b), the atomistic structure along with the polyhedral units are shown. Two images along the same view (i.e. along the boundary-plane normal vector, $\hat{n} = [18 \, 9 \, 8]$) are provided to simplify the presentation.  The long orange units are repeated in the two views.  The vector $\vec{t}_1 = [5 \, \overline{2} \, \overline{9}]$ and $\vec{t}_2 = [1 \, \overline{2}\, 0]$.  This GB is close in orientation to the $\Sigma3 (111)$ GB, and hence, contains twin facets (represented by the green dual-tetrahedral units). The GB also has the CTP units that correspond to the polyhedral units of the $\Sigma 3 (2\, \overline{1}\, \overline{1})$ GB.  The two-dimensional unit cells of the GBs are highlighted and four unit cells are shown. The GB contains ledges and the polyhedral units that belong to these ledges are the same as those observed in the $\Sigma 3 (9\, \overline{4} \, \overline{5})$.  The blue polyhedral unit has the same structure as shown in Figure \ref{fig:s3c} with fifteen atoms. The long polyhedral unit (shown in orange) is an extension of the orange polyhedral unit shown in Figure \ref{fig:s3c}. The polyhedral units of the ledge are emphasized in (c) by viewing the GB along the $[0 \, 1 \, \overline{1}]$ axis.}
  \label{fig:s3d}
\end{figure}


\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.9]{s49_topview_aftersplit.png}
  % \includegraphics[width=\linewidth]{Numbered_Figures/Figure_8.png}
  \caption{\colb{The polyhedral unit model of the $\Sigma 49 a (450 \, 221 \, 113) (\bar{9} \, \bar{2} \, \bar{5})$ general GB is illustrated. The units shown here are those obtained after the post-processing analysis described in section \CBred{S4.2} of the Supplementary Information. The unit-cell of the GB is described by vectors $\vec{t}_1 = [\overline{5} \, 2 \, 16]$ and $\vec{t}_2 = [\overline{16} \, 29 \, 7]$. The boundary-normal vector along which the GB is viewed in this figure is $\hat{n} = [\overline{450} \, \overline{221} \, \overline{113}]$. The two-dimensional unit cells of the GBs are highlighted. For the sake of simplicity, only units with greater than seven atoms are shown in this figure.}}
  \label{fig:s49}
\end{figure}


\begin{figure}[h]
  \centering
  % \includegraphics[scale=0.75]{atom_shuff.png}
  % \includegraphics[scale=0.75]{Numbered_Figures/Figure_9.png}
  \caption{In (a) and (b), the polyhedral unit models of the GB structures of $\Sigma 3 (2 \overline{1} \overline{1})$ and $\Sigma 3 (13 \, \overline{5} \, \overline{5})$, respectively, are shown as viewed along the boundary-plane normal. The polyhedral units that belong to the GB unit-cell are highlighted and the basis-vectors of the unit-cell are also shown using dashed-blued lines. It is evident that the structures of these two GBs are similar except for a shift in one of the CTP units. The shift vector is crystallographically equivalent to the burgers vector $\vec{b} = \frac{a}{2} [1 \, \overline{1} \, 0]$. In order to emphasize the similarity in the GB structures, an illustration of the two GBs overlapping on each other is provided in (c). The view in (c) is along the $[0 \, 1 \,\overline{1}]$ lattice direction.}
  \label{fig:shuff}
\end{figure}







